Isotopies of Legendrian 1-knots and Legendrian 2-tori

We construct a Legendrian 2-torus in the 1-jet space of $S^1\times\R$ (or of $\R^2$) from a loop of Legendrian knots in the 1-jet space of $\R$. The differential graded algebra (DGA) for the Legendrian contact homology of the torus is explicitly computed in terms of the DGA of the knot and the monodromy operator of the loop. The contact homology of the torus is shown to depend only on the chain homotopy type of the monodromy operator. The construction leads to many new examples of Legendrian knotted tori. In particular, it allows us to construct a Legendrian torus with DGA which does not admit any augmentation (linearization) but which still has non-trivial homology, as well as two Legendrian tori with isomorphic linearized contact homologies but with distinct contact homologies.

==> Sec/chmap.tex <==
\section{Chain isomorphisms}
\label{S:chiso}

In this section we give an algebraic proof of the fact that the contact homologies of the tori constructed as isotopy traces depend only on the chain homotopy class of the chain maps of the isotopy. In fact we show something slightly more general: two contact homology algebras constructed from chain homotopic chain maps are tame isomorphic.

Let $L_+$ and $L_-$ be Legendrian links with contact homology algebras $(\A_+,\pa_+)$ and $(\A_-,\pa_-)$, respectively. Let $\phi\colon \A_+\to\A_-$ and $\psi\colon\A_+\to\A_-$ be chain maps and let $K\colon \A_+\to\A_-$ be a chain homotopy between them. That is,
\[
\phi+\psi=K\circ\pa_+ + \pa_-\circ K.
\]
Consider the DGA $\A$ generated by $\hat \A_+$, $\A_+$, and $\A_-$ with the two differentials
$\Delta_\phi\colon\A\to\A$ and $\Delta_\psi\colon\A\to\A$ defined as follows on generators
\begin{align*}
\Delta_\phi(c)=\Delta_\psi(c)=\pa_+(c),\qquad &c\in\A_+,\\
\Delta_\phi(v)=\Delta_\psi(v)=\pa_-(v),\qquad &v\in\A_-,\\
\Delta_\phi(\hat c)= c + \phi(c) +\Gamma_\phi(\pa_+(c)),\qquad &\hat c\in\hat \A_+,\\
\Delta_\psi(\hat c)= c + \psi(c) +\Gamma_\psi(\pa_+(c)),\qquad &\hat c\in\hat \A_+.
\end{align*}

Define the map $\Gamma_K\colon \A_+\to\A$ to equal zero on constants and on linear monomials and by the following expression for monomials $b_1\dots b_r$ of length $r\ge 2$ 
\[
\Gamma_K(b_1\dots b_r) = \hat b_1 K(b_2\dots b_r) + b_1\hat b_2 K(b_3\dots b_r) + \dots +
b_1\dots b_{r-2}\hat b_{r-1}K(b_r).
\]

\begin{lma}
The algebra map $F\colon (\A,\Delta_\phi)\to (\A,\Delta_\psi)$ defined on generators as follows
\begin{align*}
F(c)=c, &\qquad c\in\A_+,\\
F(v)=v, &\qquad v\in\A_-,\\
F(\hat c)=\hat c + K(c) + \Gamma_K(\pa_+ c), &\qquad c\in\hat\A_+,
\end{align*}
is a (tame) chain isomorphism. That is,
\[
F\circ\Delta_\phi=\Delta_\psi\circ F.
\]
\end{lma}

\begin{pf}
In order to facilitate computations we introduce the following notation. Let $H\colon\A_+\to\A$ and $\theta\colon \A_+\to A$ be maps. Then define the map $\Omega_\theta^{H}\colon\A_+\to\A$ as follows on monomials
\[
\Omega_\theta^{H}(b_1\dots b_r)= H(b_1)\theta(b_2\dots b_r) + b_1 H(b_2)\theta(b_3\dots b_r) + \dots + b_1\dots b_{r-1}H(b_r).
\] 
We compute
\begin{align}\label{e:comp1}
F(\Delta_\phi(\hat c)) &=
F(c + \phi(c) + \Gamma_\phi(\pa_+ c))\\\notag
&=c + \phi(c) + \Gamma_\phi(\pa_+ c) + \Omega_\phi^{K}(\pa_+ c) + \Omega_\phi^{\Gamma_K\circ\pa_+}(\pa_+ c),
\end{align}
and
\begin{align}\label{e:comp2}
\Delta_\psi(F(\hat c)) &=
\Delta_\psi(\hat c + K(c) + \Gamma_K(\pa_+ c))\\\notag
&=c + \psi(c) + \Gamma_\psi(\pa_+ c) + \pa_-(K(c)) + \Delta_\psi(\Gamma_K(\pa_+ c)).
\end{align}
We note that the monomials in \eqref{e:comp1} and \eqref{e:comp2} are of two types: monomials which are constant in $\hat\A_+$-generators and monomials which are linear in $\hat\A_+$-generators. We first show that the monomials of the former kind cancels between the two equations. 

The contribution from \eqref{e:comp1} to monomials of the first kind is 
\[
c+\phi(c)+\Omega_\phi^{K}(\pa_+ c)
\] 
and the contribution from \eqref{e:comp2} is
\[
c+\psi(c)+\pa_-(K(c))+\Delta_\psi(\Gamma_K(\pa_+ c))_0,
\]
where $w_0$ denotes the term in an element which is constant in the $\hat\A_+$-genetartors.
Thus, if we show that 
\begin{equation}\label{e:monomial1}
\Omega_\phi^{K}(\pa_+ c)+\Delta_\psi(\Gamma_K(\pa_+ c))_0=K(\pa_+ c)
\end{equation}
then it follows that monomials of the first type cancels. Now, if $b_1\dots b_r$ is a monomial in $\pa_+ c$ then the contribution from this monomial to the left hand side of \ref{e:monomial1} which is non-constant in the $\A_+$-generators vanishes for the following reason. Terms arising from $\Omega_\phi^{K}$ have the form
\[
b_1\dots b_s K(b_{s+1})\phi(b_{s+2})\dots\phi(b_r)
\]
and are canceled by terms in $\Delta_\psi(b_1\dots \hat b_s K(b_{s+1})\phi(b_{s+2})\dots\phi(b_{r}))$ corresponding to the $b_s$-term in $\Delta_\psi(\hat b_s)$. Remaining terms in $\Delta_\psi(b_1\dots \hat b_s K(b_{s+1}\dots b_{r}))$ corresponding to the $b_s$-term in $\Delta_\psi(\hat b_s)$ cancels with terms in $\Delta_\psi(b_1\dots b_s\hat b_{
s+1} K(b_{s+2}\dots b_r))$ corresponding to the $\psi(b_{s+1})$-term in $\Delta_\psi(\hat b_{s+1})$. Thus if $b_1\dots b_r$ is any monomial in $\pa_+ c$ then its contribution to the left hand side of \eqref{e:monomial1} is exactly
\[
K(b_1)\phi(b_2)\dots\phi(b_r)+\psi(b_1)K(b_2)\phi(b_3)\dots\phi(b_r)+\dots \psi(b_1)\dots\psi(b_{r-1})K(b_r)
\]
and \eqref{e:monomial1} follows.

We next consider monomials linear in $\hat\A_+$-generators contributing to \eqref{e:comp1} and \eqref{e:comp2}. To this end we define the maps $A,B,C,D\colon\A_+\to\A$ as follows on monomials. 
\begin{align*}
A(b_1\dots b_s)&=\Gamma_\psi(\pa_+ b_1)K(b_2\dots b_s)\\
&+b_1\Gamma_\psi(\pa_+b_2)K(b_3\dots b_s)+\dots\\
&+b_1\dots b_{s-2}\Gamma_\psi(b_{s-1})K(b_s),
\end{align*}
if $s\ge 2$ and $0$ otherwise.
\begin{align*}
B(b_1\dots b_s)&=\hat b_1K(\pa_+(b_2\dots b_s))\\
&+b_1\hat b_2K(\pa_+(b_3\dots b_s))+\dots\\
&+b_1\dots b_{s-2}\hat b_{s-1}K(\pa_+(b_s)),
\end{align*}
if $s\ge 2$ and $0$ otherwise.
\begin{align*}
C(b_1\dots b_s)&=(\pa_+ b_1)\hat b_2K(b_3\dots b_s)\\
&+\pa_+(b_1b_2)\hat b_3K((b_4\dots b_s))+\dots\\
&+\pa(b_1\dots b_{s-2})\hat b_{s-1}K(b_s),
\end{align*}
if $s\ge 2$ and $0$ otherwise.
\begin{align*}
D(b_1\dots b_s)&=\hat b_1\pa_-(K(b_2\dots b_s))\\
&+b_1\hat b_2\pa_-(K(b_3\dots b_s))+\dots\\
&+b_1\dots b_{s-2}\hat b_{s-1}\pa_-(K(b_s)),
\end{align*}
if $s\ge 2$ and $0$ otherwise.

We have
\[
0=\Gamma_K(\pa_+\pa_+ c)=\Omega^{\Gamma_K\circ\pa_+}(\pa_+ c) + A(\pa_+ c) + B(\pa_+ c) + C(\pa_+ c).
\]
(To see this one subdivides contributing monomials as follows. Let $b_1\dots b_s$ be a monomial in $\pa_+c$. The first term corresponds to the $\hat \A_+$-variable and the $K$-variable both located in a $\pa b_j$-monomial some $j$. The second term corresponds to the $\hat\A_+$-variable in a $\pa b_j$-monomial and the $K$-variable outside. The third term corresponds to the $\hat \A_+$-variable outside a $\pa_+ b_j$-monomial and the variable on which the $\pa_+$-operator acts being on the right of the $\hat \A_+$-generator. The fourth term corresponds to the $\hat \A_+$-variable outside a $\pa_+ b_j$-monomial and the variable on which the $\pa_+$-operator acts being on the left of the $\hat \A_+$-generator.)
 
Similarly, we have
\[
\Delta_\psi(\Gamma_K(\pa_+ c))_1= A(\pa_+ c) + C(\pa_+ c)+ D(\pa_+ c),
\]
where $w_1$ denotes the term of an element which is linear in the $\hat\A_+$-generators. Consequently, the contribution of monomials of the second kind to the sum of \eqref{e:comp1} and \eqref{e:comp2} is
\begin{align*}
&\Gamma_\phi(\pa_+ c)+\Gamma_\psi(\pa_+ c)+\Omega^{\Gamma_K\circ\pa_+}(\pa_+ c)+\Delta_\psi(\Gamma_K(\pa_+ c))_1\\
&=\Gamma_\phi(\pa_+ c)+\Gamma_\psi(\pa_+ c)+ B(\pa_+c) + D(\pa_+ c)=0.
\end{align*}
The lemma follows.
\end{pf}


